Fourier Sliced-Wasserstein Embedding for Multisets and Measures

We present the Fourier Sliced-Wasserstein (FSW) embedding - a novel method to embed multisets and measures over R^d into Euclidean space. Our proposed embedding approximately preserves the sliced Wasserstein distance on distributions, thereby yielding geometrically meaningful representations that better capture the structure of the input. Moreover, it is injective on measures and bi-Lipschitz on multisets - a significant advantage over prevalent methods based on sum- or max-pooling, which are provably not bi-Lipschitz, and, in many cases, not even injective. The required output dimension for these guarantees is near-optimal: roughly 2Nd, where N is the maximal input multiset size. Furthermore, we prove that it is impossible to embed distributions over R^d into Euclidean space in a bi-Lipschitz manner. Thus, the metric properties of our embedding are, in a sense, the best possible. Through numerical experiments, we demonstrate that our method yields superior multiset representations that improve performance in practical learning tasks. Specifically, we show that (a) a simple combination of the FSW embedding with an MLP achieves state-of-the-art performance in learning the (non-sliced) Wasserstein distance; and (b) replacing max-pooling with the FSW embedding makes PointNet significantly more robust to parameter reduction, with only minor performance degradation even after a 40-fold reduction.

==> base/packages.tex <==
% Neat and Flexible LaTeX Template
% Written by Tal Amir 2024
% https://tal-amir.github.io/
%
% File: base/packages.tex
% to be loaded from base/base.tex
%
% This file is for loading packages and setting settings related to those packages.
% Math-related macros are loaded from base/math.tex


%\RequirePackage[utf8]{inputenc} % allow utf-8 input
\RequirePackage[T3,T1]{fontenc}  % load T1 and T3 font encodings
\RequirePackage{hyperref}        % hyperlinks
\RequirePackage{url}             % simple URL typesetting
%\RequirePackage{amsfonts}       % blackboard math symbols
\RequirePackage{nicefrac}        % compact symbols for 1/2, etc.
%\RequirePackage{microtype}      % microtypography
\RequirePackage{xcolor}
%\RequirePackage{color}
%\RequirePackage{colortbl}       % used for \cellcolor
\RequirePackage{float}
\RequirePackage{threeparttable}
%\RequirePackage{floatrow}        % for \floatfoot. does not work with the float package
\RequirePackage{nicematrix}      % For the NiceTabular table environment
\RequirePackage{booktabs}        % professional-quality tables
\RequirePackage{multirow}        % gives better control over vertical alignment than \Block[c]{2-1}{xxx}
\RequirePackage{wrapfig}
%\RequirePackage{subcaption}     % allows adding captions to subfigures
\RequirePackage{graphicx}
%\RequirePackage{enumerate}      % for roman numerals
\RequirePackage{extarrows}
\RequirePackage{etoolbox}
\RequirePackage{ifthen}         % provides \ifthenelse
\RequirePackage{apptools}       % provides \IfAppendix
\RequirePackage{lineno}         % provide nolinenumbers environment

%  ----------------------- 
% ---- siunitx package ----
%  ----------------------- 
% Enables controlling the appearance of captions
\RequirePackage{caption}
%\RequirePackage[font=small,labelfont=bf]{caption} % Make caption font size small
\captionsetup{font=small}
%\captionsetup[table]{skip=10pt}


%  ----------------------- 
% --- pgfplots and tikz ---
%  ----------------------- 
\RequirePackage{pgfplots}
\pgfplotsset{width=6cm,compat=newest} 
\usepgfplotslibrary{groupplots}
\usetikzlibrary{pgfplots.groupplots}

% Externalize the figures, i.e. save them to separate PDFs
\usepgfplotslibrary{external}
% Tal: This command tells Tikz to generate external PDF files with the plots.
% It produces an error when compiling with Texlive 2020 or through Arxiv's webpage. 
% In those cases it can simply be turned off, resulting in a slower compilation.
%\tikzexternalize


%  ---------------------- 
% --- cleveref package ---
%  ---------------------- 
%\RequirePackage{cleveref}
\RequirePackage[noabbrev,capitalise]{cleveref} % These options might clash with the options defined in the conference style file

% Remove the word 'equation' from references:
\crefname{equation}{}{}
%\crefrangeformat{equation}{(#3#1#4)\,--\,(#5#2#6)} % Use en-dash instead of 'to' in equation range.

% A lower-level way to remove the word 'equation' from references:
%\crefformat{equation}{(#2#1#3)}
%\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
%\crefmultiformat{equation} {(#2#1#3)} { and~(#2#1#3)} {, (#2#1#3)} { and~(#2#1#3)}


%  --------------------- 
% --- siunitx package ---
%  --------------------- 
\RequirePackage{siunitx} % for displaying percents and other units
\sisetup{detect-all, group-separator = {,}, output-decimal-marker={.}}
%\sisetup{detect-weight=true,detect-inline-weight=math}
\DeclareSIUnit{\million}{\textup{million}}
\DeclareSIUnit{\millisecond}{\milli\second} 


==> figures/fig_modelnet_shrunk_models_for_erc.tex <==
\pgfplotsset{every tick label/.append style={font=\small}}
%
\begin{figure}
\centering
%\vspace{-5mm}
\begin{tikzpicture}
\inputfigure{plot_modelnet_shrunk_models_for_erc.tex}
\end{tikzpicture}
%
%\\
%\small
%Explanation about the figure.
%
\caption{ModelNet40 classification accuracy\label{fig_modelnet_shrunk_models_for_erc}}
\end{figure}



==> figures/plot_modelnet_shrunk_models_for_erc.tex <==
\begin{semilogxaxis}[xlabel=Number of parameters,
    width=0.6\textwidth,
    %height=\textheight,
    %ylabel=Accuracy,
    ymin = 0,
    ymax = 100,
    grid = both,
    legend style={at={(0.95,0.05)},anchor=south east,draw=black,fill=white,align=left,
    nodes={scale=0.75, transform shape}},   yticklabel={\pgfmathparse{\tick*1}\pgfmathprintnumber{\pgfmathresult}\%},
    ]
    
\addplot [line width=0.5pt,solid,color=blue, solid, mark=*, mark size=1pt] table [x=num_params, y=test_accuracy, col sep=comma] {\csvpath modelnet_shrunk_models_swe.csv};
\addlegendentry{Ours} 

\addplot [line width=0.5pt,solid,color=red, solid, mark=square*, mark size=1pt] table [x=num_params, y=test_accuracy, col sep=comma] {\csvpath modelnet_shrunk_models_pointnet.csv};
\addlegendentry{PointNet} 

%\node[draw] at (3471473,85.2512) {Original size};

\end{semilogxaxis}


==> latexmkrc <==
# This is the configuration for latexmk
# Enabling write18 and shell escape for pdflatex
# This is probably needed for \tikzexternalize, not sure
$pdflatex = 'pdflatex --enable-write18 --shell-escape %O %S';


==> tables/table_empirical_distortion.tex <==
\newcommand{\oomcell}{{{\begingroup{\emph{OOM}}\endgroup}}}
\newcommand{\fixheaderheight}[1]{\raisebox{-0.6ex}{{#1}}}

\begin{table}[htb]
    \centering
    \begin{minipage}[t]{0.69\linewidth}  % Adjust width as needed
    \centering    
    \begingroup
    %
    \caption{\label{table_empirical_distortion}Empirical Distortion Evaluation}\label{tab:empirical_distortion}
    %
    \fontsize{8}{8}\selectfont
    \renewcommand*{\arraystretch}{1.05}    
    %
    % Setting the \arraystretch above 1 increases the space between cells.
    % Using \begingroup and \endgroup makes sure that the redefinition
    % of \arraystretch is only local to this table.
    \begin{NiceTabular}{ccccS[table-format=2.2]S[table-format=2.2]S[table-format=2.2]S[table-format=2.2]}
        \toprule % \Block[c]{1-1}{Dataset}
        \multirow{2}{*}{\fixheaderheight{Dataset}} & \multirow{2}{*}{\fixheaderheight{$d$}} & \multirow{2}{*}{\fixheaderheight{$n$}} & \multirow{2}{*}{\fixheaderheight{Method}} & \Block{1-4}{$m$} & & &    
    \\ \cmidrule(l{2pt}r{2pt}){5-8} & & & & \Block[c]{1-1}{10} & \Block[c]{1-1}{50} & \Block[c]{1-1}{200} & \Block[c]{1-1}{1000}
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} 
    %
    \multirow{2}{*}{ModelNet} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$2047$} & PSWE & 2.55 & 1.48 & \oomcell & \oomcell
    \\ & & & FSW & 2.57 & 1.46 & \oomcell & \oomcell
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{RNAseq} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$20$} & PSWE & 4.36 & 3.64 & \oomcell & \oomcell
    \\ & & & FSW & 4.08 & 3.48 & \oomcell & \oomcell
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$20$} & PSWE & 2.35 & 1.4 & 1.2 & \oomcell
    \\ & & & FSW & 2.18 & 1.36 & 1.16 & 1.07
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$10$} & \multirow{2}{*}{$20$} & PSWE & 2.3 & 1.47 & 1.22 & \oomcell
    \\ & & & FSW & 2.32 & 1.4 & 1.18 & 1.08
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$100$} & \multirow{2}{*}{$20$} & PSWE & 2.35 & 1.38 & 1.23 & \oomcell
    \\ & & & FSW & 2.41 & 1.43 & 1.19 & 1.08
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$1000$} & \multirow{2}{*}{$20$} & PSWE & 2.3 & 1.4 & 1.17 & \oomcell
    \\ & & & FSW & 2.45 & 1.43 & 1.19 & 1.08
    %
    \\ \bottomrule
    \end{NiceTabular}
    \endgroup
    \end{minipage}
    %
    \begin{minipage}[t]{0.3\linewidth}
    \vspace{8.6mm}
    \caption*{Empirical distortion with respect to the sliced Wasserstein distance, evaluated on real and synthetic data. In each trial, distortion was evaluated on 6000 point clouds. The numbers show the average over 200 independent trials. $d$, $n$: ambient dimension and number of points in each cloud; $m$: embedding dimension; OOM: Out of Memory---the method failed due to insufficient memory.}
    \end{minipage}
    %
\end{table}


==> text/proof_failure_of_blip_original.tex <==
\thmFailureOfBlip*

\begin{proof}\label{proof_failure_of_blip}
%
Our proof of \cref{thm_failure_of_blip} consists of three steps. First, in \cref{lemma_nonlip_A} below, we prove the theorem for the special case that $\emb$ is homogeneous and $\Omega$ is an open ball centered at zero. Then, in \cref{lemma_nonlip_B}, we release the homogeneity assumption by considering a homogenized version of $\emb$. Finally, we generalize to arbitrary $\Omega$ with a nonempty interior in a straightforward manner.

Let us begin with the special case of a homogeneous $\emb$.

\begin{lemma}\label{lemma_nonlip_A}
    Let $\emb : \Pnof\Omega \to \RR^m$, with $\Omega \subseteq \RR^d$ being an open ball centered at zero, $n \geq 2$ and $m \geq 1$. Suppose that $\emb$ is \emph{homogeneous}, i.e. $\emb\of{\alpha \mu} = \alpha \emb\of\mu$ for any $\mu \in \Pnof\Omega$, $\alpha \geq 0$. Then for all $p\in\brs{0,\infty}$, $\emb$ is not bi-Lipschitz with respect to $\Wassp$.
\end{lemma}


\begin{proof}
    %
    Let $\brc{\delta_t}_{t=1}^\infty$ be a sequence of real numbers such that
    %
    \begin{equation}\label{proof_nonlip_homogeneous_delta_descent}
        0 < \delta_{t+1} \leq \tfrac{1}{2}\delta_{t} \leq 1 \quad \forall t \geq 1.
    \end{equation}

    For a sequence $\brc{x_t}_{t=1}^\infty$ in a Euclidean space, denote by
    %
    \begin{equation*}
        \limpar_{t\to\infty} x_t
    \end{equation*}
    %
    the set of all \emph{finite} partial limits of $x_t$ as $t \to \infty$. In particular, if $x_t$ has no convergent subsequence, then $\limpar_{t\to\infty} x_t = \varnothing$.
    
    For a probability vector $\bp \in \Delta^n$, we say that $\bv \in \RR^n$ is an \emph{admissible direction} at $\bp$ if $\bp + \delta \bv \in \Delta^n$ for all small enough $\delta>0$. 
    
    Let $p\in\brs{0,\infty}$. Define $\partial^p\emb\of{\bX,\bp,\bv}$ for $\bX \in \Omega^n$, $\bp \in \Delta^n$, and $\bv \in \RR^n$ an admissible direction at $\bp$, by
    %
    \begin{equation}\label{proof_nonlip_homogeneous_seqdef}
        \partial^p\emb\of{\bX,\bp,\bv} \eqdef \limpar_{t\to\infty} \frac{ \emb\of{\bX,\bp + \delta_t \bv} - \emb\of{\bX,\bp} } {\rootp{\delta_t}},
    \end{equation}
    %
    with the convention $\rootp[\infty]{x} = 0$ for $x > 0$, which we shall use throughout this proof.
    
    Let $\mu \in \Pnof{\Omega}$ be an arbitrary distribution supported on $k$ distinct nonzero points $\bx[1],\ldots,\bx[k] \in \Omega$ with $1 \leq k<n$. Then $\mu$ can be expressed as $\mu = \sum_{i=1}^{k} p_i\delta_{\bx[i]}$ with $p_1,\ldots,p_k > 0$ and $p_1+\ldots+p_k=1$. Augment $\bx[i]$ to $k+1 \leq i \leq n$ by setting $\bx[i]=0$, and let $\bX^0 = \br{\bx[1],\ldots,\bx[n]} \in  \RR^{d \times n}$. Denote
    %
    \[ x_{\min} \eqdef \min_{i \in \brs{k}} \norm{\bx[i]}. \]
    %
    By our assumption, $x_{\min} > 0$.

    
    Let $\bp^0, \bp^1 \in \Delta^n$ be given by
    %
    \begin{equation*}
    \begin{split}
        \bp^0 &\eqdef \br{\overbrace{0,0,\ldots,0}^{\text{$k$}},\overbrace{\tfrac{1}{n-k},\ldots,\tfrac{1}{n-k}}^{n-k}}
        \\
        \bp^1 &\eqdef \br{p_1,\ldots,p_k,0,\ldots,0},
    \end{split}
    \end{equation*}
    %
    and let $\bv^1 \in \RR^n$ be the direction vector
    %
    \begin{equation*}
        \bv^1 \eqdef \bp^1-\bp^0 = \br{p_1,\ldots,p_k,\tfrac{-1}{n-k},\ldots,\tfrac{-1}{n-k}},
    \end{equation*}
    %
    which is admissible at $\bp^0$.
    Augment the definition of $\bp^0, \bp^1$ by
    %
    \begin{equation*}
    \begin{split}
        \bp^{\delta} &\eqdef \br{1-\delta}\bp^0 + \delta \bp^1 = \bp^0 + \delta \bv^1
        \quad\text{for}\quad
        \delta \in \brs{0,1}.
    \end{split}
    \end{equation*}

    
    Denote by $\mu\of{\delta}$ for $\delta \in \brs{0,1}$ the distribution parametrized by $\br{\bX^0,\bp^{\delta}}$. 
    Then $\mu\of{0}=0$ and $\mu\of{1} = \mu$. With this notion, we have that 
    %
    \begin{equation}\label{proof_nonlip_homogeneous_seqdef_X0}        
    \begin{split}
        \partial^p\emb\of{\bX^0,\bp^0,\bv^1} 
        \eqx &\limpar_{t\to\infty} \frac{ \emb\of{\bX^0,\bp^0+\delta_t \bv^1} - \emb\of{\bX^0,\bp^0} } {\rootp{\delta_t}}  
        \\ \eqx &\limpar_{t\to\infty} \frac{ \emb\of{\bX^0,\bp^{\delta_t}} - \emb\of{0} } {\rootp{\delta_t}}  
        \eqx \limpar_{t\to\infty} \frac{ \emb\of{\mu\of{\delta_t}} } {\rootp{\delta_t}},
    \end{split}
    \end{equation}

    %
    where $\emb\of{0} = 0$ holds by the homogeneity assumption.
    For all $t \geq 1$, if $p<\infty$ then
    %
    \begin{equation*}
        \Wasspp\of{ \mu\of{\delta_t}, 0 }
        =
        \sum_{i=1}^k \delta_t p_i \norm{\bx[i] - 0}^p
        =
        \delta_t \sum_{i=1}^k p_i \norm{\bx[i]}^p
        =
        \delta_t \norm{\mu}_{\Wassp}^p
        > 0,
    \end{equation*}
    %
    and if $p=\infty$, then
    %
    \begin{equation*}    
        \Wass[\infty]\of{ \mu\of{\delta_t}, 0 }
        =
        \max_{i\in\brs{k}} \norm{\bx[i] - 0}
        =
        \norm{\mu}_{\Wass[\infty]} > 0.
    \end{equation*}
    %
    Thus, in both cases, it follows from \cref{proof_nonlip_homogeneous_seqdef_X0} that
    %    
    \begin{equation}\label{proof_nonlip_homogeneous_seqdef_X0_b}
        \partial^p\emb\of{\bX^0,\bp^0,\bv^1}
        = \norm{\mu}_\Wassp \limpar_{t\to\infty} \frac{ \emb\of{\mu\of{\delta_t}} - \emb\of{0} } { \Wassp\of{ \mu\of{\delta_t}, 0 } },
    \end{equation}
    %
    with the multiplication above denoting the multiplication of the set $\limpar_{t\to\infty} \frac{ \emb\of{\mu\of{\delta_t}} - \emb\of{0} } { \Wassp\of{ \mu\of{\delta_t}, 0 } }$ by the positive scalar $\norm{\mu}_\Wassp$.

    %We now show that $\partial^p E\of{\bX^0,\bp^0,\bv^1}$ is nonempty and does not contain zero. 
    If $\partial^p E\of{\bX^0,\bp^0,\bv^1}$ is empty, then by \cref{proof_nonlip_homogeneous_seqdef_X0_b}, the sequence 
    \[
        \brc{ \frac{ \emb\of{\mu\of{\delta_t}} - \emb\of{0} } { \Wassp\of{ \mu\of{\delta_t}, 0 } } }_{t \geq 1}
        \subset \RR^m
    \]
    is unbounded, which implies that $\emb$ is not upper-Lipschitz. Similarly, if $0 \in \partial^p E\of{\bX^0,\bp^0,\bv^1}$, then the above sequence is not isolated from zero, which implies that $\emb$ is not lower-Lipschitz. Hence, in order for $\emb$ to be bi-Lipschitz, $\partial^p E\of{\bX^0,\bp^0,\bv^1}$ must be nonempty and cannot contain zero. Suppose there exists $L \in \partial^p E\of{\bX^0,\bp^0,\bv^1}$ such that $L \neq 0$.

    So far we only assumed that $\brc{\delta_t}_{t \geq 1}$ is an arbitrary sequence that satisfies \cref{proof_nonlip_homogeneous_delta_descent}. Note that property \cref{proof_nonlip_homogeneous_delta_descent} is preserved under taking subsequences. Therefore, by replacing the original $\delta_t$ with its appropriate subsequence, we can assume without loss of generality that the partial limits in \cref{proof_nonlip_homogeneous_seqdef_X0} are in fact a limit, so
    \[
        \partial^p E\of{\bX^0,\bp^0,\bv^1} = \brc{L},
    \]
    %
    and thus by \cref{proof_nonlip_homogeneous_seqdef_X0},
    %
    \begin{equation}\label{proof_nonlip_homogeneous_lim_aa}
        \lim_{t\to\infty} \frac{ \emb\of{\mu\of{\delta_t}} } {\rootp{\delta_t}} = L.
    \end{equation}
    %
    Let $\brc{e_t}_{t \geq1 } \subseteq \RR^m$ be the sequence
    %
    \begin{equation*}
        e_t \eqdef \emb\of{\mu\of{\delta_t}} - L \rootp{\delta_t}, \quad t \geq 1.
    \end{equation*}
    %
    Then
    %
    \begin{equation}\label{proof_nonlip_homogeneous_lim}
        \emb\of{\mu\of{\delta_t}} = L \rootp{\delta_t} + e_t,
        \quad
        t \geq 1,
    \end{equation}
    %
    and by \cref{proof_nonlip_homogeneous_lim_aa},
    %
    \begin{equation}\label{proof_nonlip_homogeneous_lim_et}
        \lim_{t\to\infty} \frac{e_t}{\rootp{\delta_t}} = 0.
    \end{equation}
    %
    Now consider the sequence of distributions
    \[ 
        \tilde\mu_t \eqdef \rootp{\frac{\delta_t}{\delta_{t-1}}}\mu\of{\delta_{t-1}}, \quad t\geq 2.
    \]
    Since $\frac{\delta_t}{\delta_{t-1}} \leq 1$, and $\Omega$ is a ball centered at zero, then $\bX^0 \in \Omega^n$ implies that $\rootp{\frac{\delta_t}{\delta_{t-1}}} \bX^0 \in \Omega^n$, and thus $\tilde\mu_t$ is indeed in $\Pnof\Omega$. We wish to lower-bound the $p$-Wasserstein distance from $\mu\of{\delta_t}$ to $\tilde\mu_t$ for $t \geq 2$.
    %
    Note that $\mu\of{\delta_t}$ assigns a mass of $1-\delta_t$ to $\bx=0$, whereas $\tilde\mu_t$ assigns a smaller mass of $1-\delta_{t-1}$ to $\bx=0$ and assigns the rest of the mass to points of $\ell_2$-norm at least $\rootp{\frac{\delta_t}{\delta_{t-1}}} x_{\min}$. Thus, transporting $\mu\of{\delta_t}$ to $\tilde\mu_t$ requires at least the transfer of a mass of $\br{1-\delta_t} - \br{1-\delta_{t-1}} = \delta_{t-1}-\delta_t$ a distance of at least $\rootp{\frac{\delta_t}{\delta_{t-1}}} x_{\min}$. We shall now show that this implies
    %
    \begin{equation}\label{proof_nonlip_homogeneous_wassbound}
    \begin{split}
        \Wassp\of{ \mu\of{\delta_t}, \tilde\mu_t }
        \geqx
        &  \rootp{ \br{\delta_{t-1}  - \delta_{t}} \frac{\delta_t}{\delta_{t-1}} } x_{\min}.
    \end{split}
    \end{equation}
    %
    If $p=\infty$, then \cref{proof_nonlip_homogeneous_wassbound} clearly holds.
    For $p<\infty$, let $\pi \in \Pi\of{ \mu\of{\delta_t}, \tilde\mu_t }$ be a transport plan from $\mu\of{\delta_t}$ to $\tilde\mu_t$. Then the $p$th power of the transport cost of $\pi$ is
    %
    \begin{equation*}
    \begin{split}
        & \sum_{i,j \in \brs{n}} \pi_{i,j}\norm{\bx[i]-\rootp{\frac{\delta_t}{\delta_{t-1}}}\bx[j]}^p
        \geq   
        \sum_{i>k,j\leq k} \pi_{i,j}\norm{\bx[i]-\rootp{\frac{\delta_t}{\delta_{t-1}}}\bx[j]}^p
        \\ \eqx[(a)] &
        \sum_{i>k,j\leq k} \pi_{i,j}\norm{0-\rootp{\frac{\delta_t}{\delta_{t-1}}}\bx[j]}^p
        \eqx
        \sum_{i>k,j\leq k} \pi_{i,j} \frac{\delta_t}{\delta_{t-1}} \norm{\bx[j]}^p
        \geqx 
        \frac{\delta_t}{\delta_{t-1}} \sum_{i>k,j\leq k} \pi_{i,j}x_{\min}^p
        \\ \eqx &  
        \frac{\delta_t}{\delta_{t-1}} x_{\min}^p \br{ \sum_{i\in \brs{n}, j\leq k} \pi_{i,j} - \sum_{i,j\leq k} \pi_{i,j} }
        \eqx[(b)]  
        \frac{\delta_t}{\delta_{t-1}} x_{\min}^p \br{ \sum_{j\leq k} \delta_{t-1}p_j - \sum_{i,j\leq k} \pi_{i,j} }
        \\ \geqx  &
        \frac{\delta_t}{\delta_{t-1}} x_{\min}^p \br{ \sum_{j\leq k} \delta_{t-1}p_j - \sum_{i\leq k,j\in\brs{n}} \pi_{i,j} }
        \eqx[(c)]  
        \frac{\delta_t}{\delta_{t-1}} x_{\min}^p \br{ \sum_{j\leq k} \delta_{t-1}p_j - \sum_{i\leq k} \delta_t p_i }
        \\ \eqx & 
        %\frac{\delta_t}{\delta_{t-1}} x_{\min}^p \br{ \delta_{t-1} - \delta_t } \sum_{i\leq k} p_i
        %=  
        \frac{\delta_t}{\delta_{t-1}} x_{\min}^p \br{ \delta_{t-1} - \delta_t },
    \end{split}
    \end{equation*}
    %
    where (a) is since $\bx[i]=0$ for all $i > k$ and (b)-(c) hold since $\pi\in\Pi\of{ \mu\of{\delta_t}, \tilde\mu_t }$. Thus, \cref{proof_nonlip_homogeneous_wassbound} holds.
    
    
    Now, for $t \geq 2$,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_lim2}
    \begin{gathered}        
        \emb\of{\tilde\mu_t} 
        \eqx
        \emb\of{\rootp{\frac{\delta_t}{\delta_{t-1}}} \mu\of{\delta_{t-1}}} 
        \eqx[(a)]
        \rootp{\frac{\delta_t}{\delta_{t-1}}} \emb\of{\mu\of{\delta_{t-1}}} 
        \\
        \eqx[(b)]
        \rootp{\frac{\delta_t}{\delta_{t-1}}} \br{ L \rootp{\delta_{t-1}} + e_{t-1} }
        \eqx
        L \rootp{\delta_{t}} + \rootp{\frac{\delta_t}{\delta_{t-1}}} e_{t-1},
    \end{gathered}
    \end{equation}
    %
    where (a) is by the homogeneity of $\emb$, and (b) follows from \cref{proof_nonlip_homogeneous_lim} with $t$ replaced by $t-1$.
    %
    Subtracting \cref{proof_nonlip_homogeneous_lim2} from \cref{proof_nonlip_homogeneous_lim} yields 
    %
    \begin{equation}\label{proof_nonlip_homogeneous_lim3}
        \emb\of{\mu\of{\delta_t}}
        -
        \emb\of{\tilde\mu_t} 
        =
        e_t - \rootp{\frac{\delta_t}{\delta_{t-1}}} e_{t-1},
        \quad
        \forall t\geq 2.
    \end{equation}
    %
    Finally, we have
    %
    \begin{equation*}
    \begin{split}
        & \frac{  \norm{ \emb\of{\mu\of{\delta_t}} - \emb\of{\tilde\mu_t} }  }{ \Wassp\of{ \mu\of{\delta_t}, \tilde\mu_t } }
        \leqx[(a)] 
        \frac{  \norm{ \emb\of{\mu\of{\delta_t}} - \emb\of{\tilde\mu_t} }  }{ \rootp{\br{\delta_{t-1}  - \delta_{t}} \frac{\delta_t}{\delta_{t-1}}} x_{\min}  } 
        \\ \eqx[(b)]&
        \frac{1}{x_{\min}}
        \frac{  \norm{ e_t - \rootp{\frac{\delta_t}{\delta_{t-1}}} e_{t-1} }  }
        { \rootp{\br{\delta_{t-1}  - \delta_{t}} \frac{\delta_t}{\delta_{t-1}}}  }
        =
        \frac{1}{x_{\min}}
        \frac{  \norm{ \frac{e_t}{\rootp{\delta_{t}}} - \frac{e_{t-1}}{\rootp{\delta_{t-1}}} }  }
        { \rootp{\br{\delta_{t-1}  - \delta_{t}} \frac{1}{\delta_{t-1}}}  }
        \\ \eqx &
        \frac{1}{x_{\min}}
        \frac{  \norm{ \frac{e_t}{\rootp{\delta_{t}}} - \frac{e_{t-1}}{\rootp{\delta_{t-1}}} }  }
        { \rootp{ 1  - \frac{\delta_t}{\delta_{t-1}}}  }
        \leqx[(c)] 
        \frac{\rootp{2}}{x_{\min}}
        \norm{ \frac{e_t}{\rootp{\delta_{t}}} - \frac{e_{t-1}}{\rootp{\delta_{t-1}}} } 
        \xrightarrow[t \to \infty]{} 0,
    \end{split}
    \end{equation*}
    %
    where (a) is by \cref{proof_nonlip_homogeneous_wassbound}; (b) is by \cref{proof_nonlip_homogeneous_lim3}; (c) follows from \cref{proof_nonlip_homogeneous_delta_descent}, since
    \[
        1-\tfrac{\delta_t}{\delta_{t-1}} \geq 1-\tfrac{1}{2} = \tfrac{1}{2};
    \]
    and the limit as $t\to\infty$ follows from \cref{proof_nonlip_homogeneous_lim_et}.
    Therefore, $\emb$ is not lower-Lipschitz. This concludes the proof of \cref{lemma_nonlip_A}.
    %    
\end{proof} % Proof of lemma_nonlip_A

The following lemma shows that the homogeneity assumption on $\emb$ can be released.

\begin{lemma}\label{lemma_nonlip_B}
    Let $\emb : \Pnof\Omega \to \RR^m$, with $\Omega \subseteq \RR^d$ being an open ball centered at zero, $n \geq 2$ and $m \geq 1$. Then for all $p\in\brs{1,\infty}$, $\emb$ is not bi-Lipschitz with respect to $\Wassp$.
\end{lemma}


\begin{proof}
    Let $p\in\brs{1,\infty}$ and suppose by contradiction that $\emb$ is bi-Lipschitz with constants $0 < c \leq C < \infty$,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq0a}
        c \cdot \Wassp\of{\mu,\tilde\mu}
        \leqx
        \norm{\emb\of\mu - \emb\of{\tilde\mu}}
        \leqx 
        C \cdot \Wassp\of{\mu,\tilde\mu},
        \qquad
        \forall \mu,\tilde\mu \in \Pnof\Omega.
    \end{equation}

    We can assume without loss of generality that $\emb\of 0 = 0$, since otherwise let
    \[ 
        \tilde\emb\of{\mu} \eqdef \emb\of\mu - \emb\of{0},
    \]
    then $\emb$ satisfies \cref{proof_nonlip_homogeneous_eq0a} if and only if $\tilde\emb$ satisfies \cref{proof_nonlip_homogeneous_eq0a}.
    
    We first prove an auxiliary claim.
    \begin{claim*}
        For any $\mu, \tilde\mu \in \Pnof\Omega$ with $\norm{\mu}_\Wassp = 1$ and $0 < \norm{\tilde\mu}_\Wassp \leq 1$, 
        %
        \begin{equation}\label{proof_nonlip_homogeneous_eq0}
        \begin{split}
            \norm{ \emb\of{\frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}} - \emb\of{\tilde\mu} }
            \leq
            C \cdot \br{1-\norm{\tilde\mu}_\Wassp}
            \leq
            C \cdot \Wassp\of{\mu,\tilde\mu}.
        \end{split}
        \end{equation}
    \end{claim*}
    %
    \begin{proof}
        By \cref{proof_nonlip_homogeneous_eq0a},
        %
        \begin{equation*}
            \norm{ \emb\of{\frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}} - \emb\of{\tilde\mu} }
            \leq 
            C\cdot \Wassp\of{ \frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}, \tilde\mu }.
        \end{equation*}
        %
        We shall now show that
        %
        \begin{equation*}
            \Wassp\of{ \frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}, \tilde\mu }
            \leq
            1-\norm{\tilde\mu}_\Wassp.
        \end{equation*}
        %
        Let $\tilde\mu = \sum_{i=1}^n p_i \delta_{\tilde\bx_i}$ be a parametrization of $\tilde\mu$. Consider the transport plan $\pi = \br{\pi_{ij}}_{i,j \in \brs{n}}$ from $\tilde\mu$ to $\frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}$ given by
        %
        \begin{equation*}
        \pi_{ij} =
        \begin{cases}
            p_i & i=j
            \\ 0 & i \neq j.
        \end{cases}
        \end{equation*}
        %
        By definition, $\Wassp\of{ \frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}, \tilde\mu }$ is smaller or equal to the cost of transporting $\tilde\mu$ to $\frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}$ according to $\pi$. Thus, for $p<\infty$,
        %
        \begin{equation*}
        \begin{split}
            \Wasspp\of{ \frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}, \tilde\mu }
            \leqx
            & \sum_{i=1}^n p_i \norm{\tfrac{1}{\norm{\tilde\mu}_\Wassp}\tilde\bx_i - \tilde\bx_i}^p
            \eqx 
            \sum_{i=1}^n p_i \norm{\br{\tfrac{1}{\norm{\tilde\mu}_\Wassp} - 1}\tilde\bx_i}^p
            \\ \eqx &
            \br{\tfrac{1}{\norm{\tilde\mu}_\Wassp} - 1}^p \sum_{i=1}^n p_i \norm{\tilde\bx_i}^p
            \eqx
            \br{\tfrac{1}{\norm{\tilde\mu}_\Wassp} - 1}^p \norm{\tilde\mu}^p_\Wassp
            \\ \eqx &
            \br{1 - \norm{\tilde\mu}_\Wassp}^p,
        \end{split}
        \end{equation*}
        %
        and thus
        \[
            \Wassp\of{ \frac{\tilde\mu}{\norm{\tilde\mu}_\Wassp}, \tilde\mu }
            \leqx
            \br{1 - \norm{\tilde\mu}_\Wassp}.
        \]
        Both sides of the above inequality are continuous in $p$, including at the limit $p\to\infty$. Thus, the above inequality also holds for $p=\infty$.
        %
        Now, to show that
        %
        \begin{equation*}            
            1-\norm{\tilde\mu}_\Wassp
            \leqx
            \Wassp\of{\mu,\tilde\mu},
        \end{equation*}
        %        
        note that
        %
        \begin{equation*}
        \begin{split}
            1 - \norm{\tilde\mu}_\Wassp
            =
            \norm{\mu}_\Wassp - \norm{\tilde\mu}_\Wassp
            =
            \Wassp\of{\mu,0} - \Wassp\of{\tilde\mu,0}
            \leq
            \Wassp\of{\mu,\tilde\mu},
        \end{split}
        \end{equation*}
        %
        where the last inequality is the reverse triangle inequality, since $\Wassp\of{\argdot,\argdot}$ is a metric.
        Thus, \cref{proof_nonlip_homogeneous_eq0} holds.
    \end{proof}

    Now we define the \emph{homogenized} function $\hat \emb : \Pnof\Omega \to \RR^{m+1}$ by
    %
    \begin{equation}
    \begin{cases}
        \hat \emb \of \mu
        \eqdef
        \brs{\norm{\mu}_\Wassp, \norm{\mu}_\Wassp \emb\of{\frac{\mu}{\norm{\mu}_\Wassp}}},
        &
        \mu \neq 0
        \\ 0 & \mu = 0.
    \end{cases}
    \end{equation}
    %
    Clearly $\hat\emb$ is homogeneous. By \cref{lemma_nonlip_A}, $\hat\emb$ it is not bi-Lipschitz with respect to $\Wassp$, and thus there exist two sequences of distributions $\mu_t, \tilde\mu_t \in \Pnof\Omega$, $t \geq 1$, such that
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq1}
        \frac{ \norm{ \hat\emb\of{\mu_t} - \hat\emb\of{\tilde\mu_t} } } {\Wassp\of{\mu_t,\tilde\mu_t}} \xrightarrow[t \to \infty]{} L,
    \end{equation}
    %
    with $L=0$ or $L=\infty$. Since $\hat\emb$ is homogeneous, we can assume without loss of generality that 
    %
    \begin{equation*}
        1 \eqx \norm{\mu_t}_\Wassp \geqx \norm{\tilde\mu_t}_\Wassp \quad \text{for all } t \geqx 1.
    \end{equation*}
    %
    This can be seen by dividing each $\mu_t$ and $\tilde\mu_t$ by $\max\brc{\norm{\mu_t}_\Wassp,\norm{\tilde\mu_t}_\Wassp}$ and swapping $\mu_t$ and $\tilde\mu_t$ for all $t$ for which $\norm{\mu_t}_\Wassp < \norm{\tilde\mu_t}_\Wassp$.
    %
    
    If $\tilde\mu_t = 0$ for an infinite subset of indices $t$, then redefine $\mu_t$ and $\tilde\mu_t$ to be the corresponding subsequences with those indices, and now \cref{proof_nonlip_homogeneous_eq1} reads as
    %
    \begin{equation*}
        \frac{ \norm{ \hat\emb\of{\mu_t} - \hat\emb\of{0} } } { \Wassp\of{\mu_t,0} }
        \eqx
        \frac{ \norm{ \emb\of{\mu_t} - \emb\of{0} } } { \Wassp\of{\mu_t,0} }        
        \xrightarrow[t \to \infty]{} L.
    \end{equation*}
    %
    This contradicts the bi-Lipschitzness of $\emb$. Therefore, $\tilde\mu_t=0$ at most at a finite subset of indices $t$. By skipping those indices in $\mu_t$ and $\tilde\mu_t$, we can assume without loss of generality that
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq1a}
        1
        \eqx
        \norm{\mu_t}_\Wassp
        \geqx
        \norm{\tilde\mu_t}_\Wassp > 0 \quad \text{for all } t
        \geqx
        1.
    \end{equation}
    
    Let us first handle the case $L=\infty$. The first component of $\hat\emb\of{\mu_t}-\hat\emb\of{\tilde\mu_t}$ is bounded by
    %
    \begin{equation*}
    \begin{split}
        \abs{ \norm{\mu_t}_\Wassp - \norm{\tilde\mu_t}_\Wassp } 
        =
        1 - \norm{\tilde\mu_t}_\Wassp  
        \leq
        \Wassp\of{\mu_t,\tilde\mu_t}
    \end{split}
    \end{equation*}
    %
    according to \cref{proof_nonlip_homogeneous_eq0}. Therefore, by \cref{proof_nonlip_homogeneous_eq1} combined with the fact that $\tilde\mu_t > 0\ \forall t$, we must have that
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq2}
        \frac{ \norm{ \norm{\mu_t}_\Wassp \emb\of{\frac{\mu_t}{\norm{\mu_t}_\Wassp}} - \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} } } {\Wassp\of{\mu_t,\tilde\mu_t}} \xrightarrow[t \to \infty]{} \infty.
    \end{equation}
    %
    On the other hand,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq3}
    \begin{split}
        & \norm{ \norm{\mu_t}_\Wassp \emb\of{\frac{\mu_t}{\norm{\mu_t}_\Wassp}} - \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \eqx[(a)]
        \norm{ \emb\of{\mu_t} - \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \\ \leqx[(b)] &
        \norm{ \emb\of{\mu_t} - \emb\of{\tilde\mu_t} }
        +
        \norm{ \emb\of{\tilde\mu_t} - \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        +
        \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} },
    \end{split}
    \end{equation}
    %
    where (a) holds since $\norm{\mu_t}_\Wassp=1$ and (b) is by the triangle inequality.
    We shall now bound the three above terms. 
    
    First,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq4a}
        \norm{ \emb\of{\mu_t} - \emb\of{\tilde\mu_t} }
        \leqx
        C \cdot \Wassp\of{\mu_t,\tilde\mu_t}
    \end{equation}
    %    
    by \cref{proof_nonlip_homogeneous_eq0a}.
    Second, 
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq4b}
    \begin{split}
        \norm{ \emb\of{\tilde\mu_t} - \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \leqx
        C \cdot \Wassp\of{ \mu_t, \tilde\mu_t }
    \end{split}
    \end{equation}    
    %    
    by \cref{proof_nonlip_homogeneous_eq0}.
    Lastly,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq4c}
    \begin{split}
        \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \eqx &
        \br{1-\norm{\tilde\mu_t}_\Wassp} \cdot \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - 0 }
        \\ \eqx &
        \br{1-\norm{\tilde\mu_t}_\Wassp} \cdot \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - \emb\of{0} }
        \\ \leqx[(a)] &
        \br{1-\norm{\tilde\mu_t}_\Wassp} \cdot C \cdot \Wassp\of{ \frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}, 0}
        \\ \eqx &
        \br{1-\norm{\tilde\mu_t}_\Wassp} \cdot C \cdot \norm{ \frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp} }_\Wassp
        \\ \eqx &
        C \cdot \br{1-\norm{\tilde\mu_t}_\Wassp}
        \leqx[(b)]
        C \cdot \Wassp\of{ \mu_t, \tilde\mu_t },
    \end{split}
    \end{equation}
    %
    where (a) is by \cref{proof_nonlip_homogeneous_eq0a} and (b) is by \cref{proof_nonlip_homogeneous_eq0}.
    %
    Inserting \cref{proof_nonlip_homogeneous_eq4a}-\cref{proof_nonlip_homogeneous_eq4c} into \cref{proof_nonlip_homogeneous_eq3} yields
    %
    \begin{equation*}
        \norm{ \norm{\mu_t}_\Wassp \emb\of{\frac{\mu_t}{\norm{\mu_t}_\Wassp}} - \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \leqx
        3 C \cdot \Wassp\of{ \mu_t, \tilde\mu_t },
    \end{equation*}
    %
    which contradicts \cref{proof_nonlip_homogeneous_eq2}.

    Let us now handle the case $L=0$.
    For two sequences of numbers $a_t,b_t \in \RR$, $t \geq 1$, we say that
    %
    \begin{equation*}
        a_t = o\of{b_t}
    \end{equation*}
    %
    if
    %
    \begin{equation*}
        \lim_{t\to\infty} \frac{a_t}{b_t} = 0.
    \end{equation*}
    %
    Denote
    %
    \begin{equation*}
        d_t
        \eqdef
        \Wassp\of{\mu_t,\tilde\mu_t}.
    \end{equation*}
    %
    According to \cref{proof_nonlip_homogeneous_eq1} with $L=0$, the first component of $\hat\emb\of{\mu_t} - \hat\emb\of{\tilde\mu_t}$, which equals $\norm{\mu_t}_\Wassp - \norm{\tilde\mu_t}_\Wassp$, satisfies
    %
    \begin{equation*}
        %\frac{1 - \norm{\tilde\mu_t}_\Wassp}{\Wassp\of{\mu_t,\tilde\mu_t}} =
        \frac{\abs{ \norm{\mu_t}_\Wassp - \norm{\tilde\mu_t}_\Wassp }}{\Wassp\of{\mu_t,\tilde\mu_t}} \xrightarrow[t \to \infty]{} 0,
    \end{equation*}
    %
    and thus
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq5z}
        1 - \norm{\tilde\mu_t}_\Wassp = \abs{ \norm{\mu_t}_\Wassp - \norm{\tilde\mu_t}_\Wassp }
        \eqx 
        o\of{d_t}.
    \end{equation}
    %
    By the triangle inequality,
    %
    \begin{gather}\label{proof_nonlip_homogeneous_eq5abcd}
    %\begin{split}        
        \norm{ \emb\of{\mu_t} - \emb\of{\tilde\mu_t} }
        \leqx
        \\ 
        \norm{ \emb\of{\mu_t} - \norm{\tilde\mu_t}_\Wassp\emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        +
        \norm{ \norm{\tilde\mu_t}_\Wassp\emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} -  \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        + 
        \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - \emb\of{\tilde\mu_t} }.
    %\end{split}
    \end{gather}
    %
    We shall show that each of the three above terms is $o\of{d_t}$. 

    First, since $\norm{\mu_t}_\Wassp=1$,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq5a}
    \begin{split}
        \norm{ \emb\of{\mu_t} - \norm{\tilde\mu_t}_\Wassp\emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \eqx &
        \norm{ \norm{\mu_t}_\Wassp \emb\of{\frac{\mu_t}{\norm{\mu_t}_\Wassp}} - \norm{\tilde\mu_t}_\Wassp\emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \\ \eqx &
        \norm{ \hat\emb\of{\mu_t} - \hat\emb\of{\tilde\mu_t} },
    \end{split}
    \end{equation}
    %
    which is $o\of{d_t}$ by \cref{proof_nonlip_homogeneous_eq1}. For the second term,
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq5b}
    \begin{split}        
        &\norm{ \norm{\tilde\mu_t}_\Wassp \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} -  \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \\ \eqx &
        \br{1 - \norm{\tilde\mu_t}_\Wassp}
        \cdot \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} }
        \\ \eqx &
        \br{1 - \norm{\tilde\mu_t}_\Wassp}
        \cdot \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - 0}
        \\ \leqx[(a)] &
        \br{1 - \norm{\tilde\mu_t}_\Wassp}
        \cdot C \cdot \Wass\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}, 0}
        \\
        \eqx &
        \br{1 - \norm{\tilde\mu_t}_\Wassp}
        \cdot C \cdot \norm{ \frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp} }_\Wassp
        \\ \eqx &
        \br{1 - \norm{\tilde\mu_t}_\Wassp}
        C 
        \eqx[(b)]
        o\of{d_t},
    \end{split}
    \end{equation}
    %
    where (a) is by \cref{proof_nonlip_homogeneous_eq0a} and (b) is by \cref{proof_nonlip_homogeneous_eq5z}.
    %
    
    Finally, by \cref{proof_nonlip_homogeneous_eq0},
    %
    \begin{equation}\label{proof_nonlip_homogeneous_eq5c}
    \begin{split}
        \norm{ \emb\of{\frac{\tilde\mu_t}{\norm{\tilde\mu_t}_\Wassp}} - \emb\of{\tilde\mu_t} }
        \leqx        
        C \cdot \br{1-\norm{\tilde\mu_t}_\Wassp}
        \eqx
        o\of{d_t}.
    \end{split}
    \end{equation}
    %
    Therefore, by \cref{proof_nonlip_homogeneous_eq5a}-\cref{proof_nonlip_homogeneous_eq5c} and \cref{proof_nonlip_homogeneous_eq5abcd}, we have that
    %
    \begin{equation*}
        \norm{ \emb\of{\mu_t} - \emb\of{\tilde\mu_t} }
        \eqx
        o\of{d_t},
    \end{equation*}
    %
    and thus $\emb$ is not lower-Lipschitz. 
    This concludes the proof of \cref{lemma_nonlip_B}.
    %
\end{proof} % Proof of lemma_nonlip_B

To finish the proof of \cref{thm_failure_of_blip}, suppose that $\Omega \subseteq \RR^d$ is an arbitrary set with a nonempty interior. Let $\Omega_0 \subseteq \Omega$ be an open ball contained in $\Omega$, and let $\bx_0$ be the center of $\Omega_0$. Then $\Omega_0-\bx_0$ is an open ball centered at zero. 

Given $\emb:\Pnof\Omega \to \RR^m$ with $n \geq 2$, define $\tilde\emb:\Pnof{\Omega_0-\bx_0} \to \RR^m$ by
%
\[
    \tilde\emb\of{\mu} \eqdef \emb\of{\mu+\bx_0}.
\]
%
Then $\tilde\emb$ satisfies the assumptions of \cref{lemma_nonlip_B}, and thus there exist two sequences of distributions $\mu_t, \tilde\mu_t \in \Pnof{\Omega_0-x_0}$, $t \geq 1$ such that
%
\begin{equation*}
    \frac{ \norm{ \tilde\emb\of{\mu_t} - \tilde\emb\of{\tilde\mu_t} } }{\Wassp\of{\mu_t,\tilde\mu_1}} 
    \xrightarrow[t \to \infty]{} L,
\end{equation*}
%
with $L=0$ or $L=\infty$. Note that the sequences $\brc{\mu_t+\bx_0}_{t\geq 1}$ and $\brc{\tilde\mu_t+\bx_0}_{t\geq 1}$ are in $\Pnof{\Omega_0}$ and thus in $\Pnof{\Omega}$. Since 
\[
    \Wassp\of{\mu_t+\bx_0,\tilde\mu_1+\bx_0}
    =
    \Wassp\of{\mu_t,\tilde\mu_1}, 
\]
we have that
%
\begin{equation*}
\begin{gathered}
    \frac{ \norm{ \emb\of{\mu_t+\bx_0} - \emb\of{\tilde\mu_t+\bx_0} } }{\Wassp\of{\mu_t+\bx_0,\tilde\mu_1+\bx_0}} 
    = 
    \frac{ \norm{ \emb\of{\mu_t+\bx_0} - \emb\of{\tilde\mu_t+\bx_0} } }{\Wassp\of{\mu_t,\tilde\mu_1}} 
    \\ \eqx
    \frac{ \norm{ \tilde\emb\of{\mu_t} - \tilde\emb\of{\tilde\mu_t} } }{\Wassp\of{\mu_t,\tilde\mu_1}} 
    \xrightarrow[t \to \infty]{} L,
\end{gathered}
\end{equation*}
%
which implies that $\emb$ is not bi-Lipschitz on $\Pnof{\Omega_0}$, and thus not on $\Pnof{\Omega}$.
%
\end{proof} % Proof of thm_failure_of_blip

